Extreme Scenario Selection in Day-Ahead Power Grid Operational Planning

We propose and analyze the application of statistical functional depth metrics for the selection of extreme scenarios in day-ahead grid planning. Our primary motivation is screening of probabilistic scenarios for realized load and renewable generation, in order to identify scenarios most relevant for operational risk mitigation. To handle the high-dimensionality of the scenarios across asset classes and intra-day periods, we employ functional measures of depth to sub-select outlying scenarios that are most likely to be the riskiest for the grid operation. We investigate a range of functional depth measures, as well as a range of operational risks, including load shedding, operational costs, reserves shortfall and variable renewable energy curtailment. The effectiveness of the proposed screening approach is demonstrated through a case study on the realistic Texas-7k grid.

==> tables/table_aggCosts.tex <==
\begin{table}[htb!]
    \centering
    \scriptsize
    \caption{Top 50 variable costs scenarios detection by aggregated net load filtering out the 500 scenarios with lowest AUC criteria. MBD was the most suitable depth metric detecting $90.51\%$ of the Top 50 variable cost scenarios.}
    \setlength{\tabcolsep}{5.75pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.25} % Default value: 1 
    \begin{tabular}{c|ccc|cccccccccc}
        \toprule
        Dates & \#Ext. & \#Sel. & Costs [k\$] & BD & MBD & DQ & ED & LID & ERD & HMD & RTD & ID & RPD \\
        \midrule
        2018-01-02 & 50 & 67 & 1,303,854 & 40.57 & 98.05 & 62.51 & 64.49 & 66.44 & 62.52 & 76.39 & 52.65 & 96.07 & 98.04 \\
        2018-01-20 & 50 & 67 & 510,801 & 58.53 & 96.12 & 74.63 & 76.57 & 84.55 & 76.57 & 92.25 & 62.87 & 90.21 & 98.06 \\
        2018-02-13 & 50 & 67 & 676,382 & 44.27 & 92.18 & 74.17 & 78.20 & 72.29 & 78.20 & 94.15 & 72.19 & 86.24 & 98.01 \\
        2018-02-14 & 50 & 67 & 539,167 & 37 & 98.08 & 64.97 & 58.98 & 72.96 & 58.98 & 82.70 & 47.12 & 94.19 & 88.32 \\
        2018-02-26 & 50 & 67 & 542,600 & 54.86 & 94.24 & 76.73 & 72.81 & 80.70 & 72.81 & 90.39 & 60.98 & 88.38 & 94.22 \\
        2018-03-14 & 50 & 67 & 492,583 & 48.61 & 100 & 56.62 & 62.55 & 64.58 & 62.55 & 86.29 & 48.54 & 96.06 & 88.25 \\
        2018-04-01 & 50 & 67 & 456,842 & 43.01 & 94.18 & 66.64 & 64.70 & 72.59 & 64.70 & 88.36 & 47.06 & 90.32 & 70.72 \\
        2018-04-09 & 50 & 67 & 496,553 & 38.50 & 92.21 & 58.61 & 58.68 & 56.66 & 58.68 & 72.56 & 48.90 & 84.35 & 84.37 \\
        2018-04-24 & 50 & 67 & 538,464 & 52.42 & 92.17 & 70.44 & 72.33 & 72.32 & 72.33 & 88.24 & 60.50 & 86.26 & 90.23 \\
        2018-05-10 & 50 & 67 & 495,807 & 42.53 & 86.32 & 64.60 & 64.70 & 66.73 & 66.67 & 80.52 & 64.69 & 84.29 & 94.16 \\
        2018-05-25 & 50 & 67 & 759,867 & 42.46 & 88.29 & 64.65 & 64.66 & 74.57 & 66.66 & 86.38 & 46.48 & 88.29 & 96.11 \\
        2018-06-04 & 50 & 67 & 793,897 & 42.39 & 98.05 & 64.49 & 66.34 & 74.44 & 66.34 & 86.30 & 58.46 & 98.03 & 98.04 \\
        2018-06-30 & 50 & 67 & 745,554 & 46.48 & 92.15 & 68.43 & 70.41 & 72.52 & 70.41 & 86.32 & 66.47 & 86.25 & 100    \\
        2018-07-22 & 50 & 67 & 1,028,589 & 40.21 & 90.13 & 58.20 & 58.25 & 72.28 & 58.25 & 72.28 & 66.22 & 86.14 & 92.12 \\
        2018-07-24 & 50 & 67 & 1,030,605 & 36.41 & 90.23 & 54.47 & 60.48 & 72.41 & 60.48 & 76.46 & 52.54 & 86.30 & 78.38 \\
        2018-08-08 & 50 & 67 & 966,812 & 34.29 & 86.15 & 66.31 & 64.37 & 64.27 & 64.36 & 74.30 & 66.24 & 86.12 & 94.06 \\
        2018-08-18 & 50 & 67 & 911,823 & 40.17 & 90.10 & 58.13 & 62.10 & 70.23 & 62.12 & 80.21 & 56.32 & 90.10 & 98.03 \\
        2018-09-04 & 50 & 67 & 769,017 & 38.41 & 82.20 & 62.38 & 64.40 & 62.42 & 64.40 & 68.42 & 50.50 & 78.21 & 76.30 \\
        2018-09-14 & 50 & 67 & 780,419 & 28.29 & 88.16 & 50.39 & 54.36 & 62.34 & 54.36 & 74.34 & 54.32 & 88.15 & 76.32 \\
        2018-10-02 & 50 & 67 & 702,130 & 38.39 & 78.31 & 58.28 & 60.41 & 66.54 & 60.41 & 74.44 & 54.64 & 78.31 & 78.35 \\
        2018-10-17 & 50 & 67 & 550,528 & 38 & 78.42 & 66.27 & 64.31 & 68.47 & 66.34 & 68.51 & 56.48 & 74.46 & 66.55 \\
        2018-11-02 & 50 & 67 & 483,866 & 34.46 & 84.27 & 56.44 & 52.48 & 60.47 & 52.48 & 72.50 & 56.49 & 76.37 & 86.24 \\
        2018-11-13 & 50 & 67 & 804,987 & 40.38 & 86.18 & 60.32 & 56.29 & 70.39 & 60.31 & 78.38 & 46.42 & 84.15 & 92.15 \\
        2018-12-01 & 50 & 67 & 364,434 & 48.63 & 96.11 & 60.72 & 68.51 & 76.55 & 68.51 & 90.37 & 52.71 & 90.18 & 96.15 \\
        2018-12-27 & 50 & 67 & 463,614 & 38.51 & 94.15 & 66.63 & 60.67 & 76.48 & 62.63 & 90.27 & 62.67 & 88.25 & 98.07 \\
        \midrule
        Med. & 50 & 67 & 676,382.97 & 40.38 & 92.15 & 64.49 & 64.37 & 72.28 & 64.36 & 80.52 & 56.32 & 86.30 & 92.15 \\
        Avg. & 50 & 67 & 688,368.38 & 41.91 & 90.66 & 63.44 & 64.08 & 70.17 & 64.48 & 81.25 & 56.50 & 87.03 & 89.25 \\
        \bottomrule
    \end{tabular}
    \label{sm:aggCosts}
\end{table}


==> tables/table_aggZonalCurtail.tex <==
\begin{table*}[htb!]
    \centering
    \small
    \caption{Total VRE curtailment detection by Far West, North Central, South Central, and West load with no filtering, and not using adaptive selection. DQ was the most suitable depth metric detecting 21.54\% of the VRE curtailment. The DQ method performs best ( 62.14\%, see in Table~SM\ref{sm:aggZonalCurtail_short}) when implementing the seasonal approach only in the days defined as extreme and filtering 450 scenarios by AUC in summer and spring season.}
    \setlength{\tabcolsep}{2.5pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.} % Default value: 1 
    \begin{tabular}{c|rrr|rrrrrrrr}
    \toprule
    \textbf{Dates} &  $|{\cal E}_k|$ & $|{\cal O}_k|$ & \textbf{GWh} & \textbf{ID} & \textbf{MBD} & \textbf{EXD} & \textbf{ERD} & \textbf{LID} & \textbf{HMD} & \textbf{DQ} & \textbf{RTD} \\
    \midrule
    2018-01-02 & 68 & 76 & 22.26 & 6.81 & 6.81 & 2.97 & 2.97 & 6.69 & 7.44 & 5.88 & 4.51 \\
    2018-01-20 & 518 & 76 & 319.39 & 29.14 & 29.28 & 28.21 & 28.00 & 11.19 & 7.52 & 9.12 & 20.50 \\
    2018-02-13 & 95 & 76 & 76.21 & 3.21 & 3.66 & 14.86 & 14.86 & 23.29 & 20.94 & 24.07 & 14.21 \\
    2018-02-14 & 771 & 76 & 772.37 & 54.65 & 51.91 & 55.48 & 55.08 & 37.51 & 31.55 & 40.65 & 45.79 \\
    2018-02-26 & 13 & 76 & 3.12 & 0.00 & 0.00 & 0.16 & 0.16 & 0.37 & 0.18 & 0.00 & 0.18 \\
    2018-03-14 & 87 & 76 & 35.79 & 6.50 & 6.60 & 5.09 & 4.69 & 5.62 & 5.19 & 6.09 & 7.01 \\
    2018-04-01 & 61 & 76 & 21.98 & 2.00 & 1.34 & 2.40 & 2.33 & 2.44 & 3.38 & 3.94 & 2.59 \\
    2018-04-09 & 33 & 76 & 13.61 & 2.67 & 2.67 & 1.84 & 1.84 & 5.41 & 3.25 & 5.98 & 1.52 \\
    2018-04-24 & 118 & 76 & 36.84 & 5.40 & 4.91 & 4.13 & 4.13 & 3.75 & 4.03 & 2.57 & 6.21 \\
    2018-05-10 & 289 & 76 & 122.20 & 12.08 & 12.39 & 8.97 & 9.79 & 11.33 & 9.92 & 10.73 & 8.80 \\
    2018-05-25 & 29 & 76 & 54.00 & 39.80 & 39.80 & 49.29 & 49.69 & 52.95 & 52.95 & 52.95 & 50.38 \\
    2018-06-04 & 17 & 76 & 26.55 & 20.18 & 20.18 & 26.55 & 26.55 & 26.55 & 26.55 & 26.55 & 26.55 \\
    2018-06-30 & 19 & 76 & 37.51 & 27.56 & 25.90 & 36.12 & 36.12 & 37.51 & 37.51 & 37.51 & 37.51 \\
    2018-07-22 & 36 & 76 & 38.30 & 30.08 & 30.08 & 33.69 & 33.69 & 36.64 & 36.64 & 36.64 & 36.75 \\
    2018-07-24 & 17 & 76 & 36.64 & 20.39 & 24.64 & 36.16 & 34.78 & 36.64 & 36.64 & 36.64 & 36.64 \\
    2018-08-08 & 15 & 76 & 21.15 & 7.75 & 7.75 & 20.80 & 20.80 & 21.15 & 21.15 & 21.15 & 20.85 \\
    2018-08-18 & 0 & 76 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    2018-09-04 & 0 & 76 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    2018-09-14 & 0 & 76 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    2018-10-02 & 4 & 76 & 1.03 & 0.70 & 0.70 & 1.03 & 1.03 & 0.82 & 0.82 & 0.82 & 0.82 \\
    2018-10-17 & 39 & 76 & 9.96 & 5.64 & 5.64 & 6.60 & 6.60 & 6.50 & 6.59 & 6.86 & 5.95 \\
    2018-11-02 & 601 & 76 & 288.86 & 28.94 & 29.45 & 35.19 & 35.19 & 38.71 & 34.91 & 36.62 & 33.92 \\
    2018-11-13 & 77 & 76 & 86.69 & 52.51 & 54.21 & 53.55 & 53.55 & 68.26 & 67.65 & 68.88 & 54.22 \\
    2018-12-01 & 49 & 76 & 15.77 & 7.19 & 7.44 & 6.95 & 6.95 & 7.91 & 7.68 & 7.38 & 6.55 \\
    2018-12-27 & 82 & 76 & 20.43 & 2.04 & 2.04 & 1.85 & 1.85 & 1.24 & 1.41 & 2.93 & 2.40 \\
    \midrule
    \textbf{Total [GWh]} & 3038 & 1900 & 2060.67 & 365.26 & 367.40 & 431.89 & 430.65 & 442.47 & 423.90 & \textbf{443.95} & 423.86 \\
    \textbf{Avg. [GWh]} & 121.52 & 76 & 82.43 & 14.61 & 14.70 & 17.28 & 17.23 & 17.70 & 16.96 & \textbf{17.76} & 16.95 \\
    \textbf{Accuracy [\%]} & - & - & - & 17.73 & 17.83 & 20.96 & 20.90 & 21.47 & 20.57 & \textbf{21.54} & 20.57 \\
    \bottomrule
    \end{tabular}
    \label{sm:aggZonalCurtail}
\end{table*}


==> tables/table_aggZonalCurtail_v0.tex <==
\begin{table}[htb!]
    \centering
    \small
    \caption{Accuracy of VC detection using selected functional depth metrics. We select $n_2(k)= |{\cal O}_k| $ scenarios based on aggregated VRE generation threshold across the 18 test days. $|{\cal E}_k|$ is the number of scenarios with realized LS and GWh refers to the total magnitude of load shedding (across scenarios) on that day. We first screen We select scenarios by using functional depth joinltly on grid-wide load and Far West zonal load.
    %Total VRE curtailment detection by aggregated load and Far West load with no filtering, and using adaptive sample number selection by aggregated total VRE generation threshold. DQ was the most suitable depth metric detecting $70.5\%$ of the VRE curtailment.}
    \setlength{\tabcolsep}{2.5pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.} % Default value: 1 
    \begin{tabular}{c|rrr|rrrrrrrr}
    \toprule
    \textbf{Dates} & $|{\cal E}_k|$ & $|{\cal O}_k|$ & \textbf{GWh} & \textbf{BD} & \textbf{MBD} & \textbf{DQ} & \textbf{EXD} & \textbf{LID} & \textbf{ERD} & \textbf{HMD} & \textbf{RTD} & \textbf{ID} & \textbf{RPD} \\
    \midrule
    2018-01-02 & 501 & 30 & 31.53 & 1 & 0.92 & 1.50 & 0.97 & \textbf{1.57} & 0.99 & 1.48 & 1.09 & 0.92 & 0.82 \\
    2018-01-20 & 578 & 1000 & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} & \textbf{321.85} \\
    2018-02-13 & 115 & 30 & 76.97 & 5.41 & \textbf{8.52} & 3.81 & 5.14 & 3.96 & 4.11 & 4.39 & 5.06 & \textbf{8.52} & 3.75 \\
    2018-02-14 & 801 & 887 & 773.98 & 677.12 & 676.89 & \textbf{688.51} & 681.82 & 677.03 & 682.22 & 665.87 & 678.97 & 678.45 & 679.54 \\
    2018-02-26 & 318 & 34 & 7.35 & \textbf{0.30} & 0.08 & 0.16 & \textbf{0.30} & 0.08 & \textbf{0.30} & 0.08 & 0.09 & 0.08 & 0.07 \\
    2018-03-14 & 129 & 229 & 37.93 & 13.21 & \textbf{17.01} & 11.97 & 12.62 & 9.84 & 12.39 & 12.45 & 10.88 & 14.78 & 13.61 \\
    2018-04-01 & 79 & 187 & 22.59 & 5.38 & 4.23 & 4.28 & 4.05 & \textbf{6.25} & 3.53 & 5.33 & 5.10 & 4.04 & 5.57 \\
    2018-04-09 & 36 & 31 & 13.69 & 0.29 & \textbf{1.56} & 0.86 & 0.62 & 0.87 & 0.28 & 1.34 & 1.22 & 0.62 & 1.01 \\
    2018-04-24 & 191 & 66 & 39.89 & 5.68 & 4.68 & 4.90 & 5.98 & 4.06 & \textbf{6.02} & 4.17 & 3.87 & 4.60 & 4.78 \\
    2018-05-10 & 368 & 1000 & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} & \textbf{126.12} \\
    2018-05-25 & 40 & 893 & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} & \textbf{54.30} \\
    2018-06-04 & 22 & 197 & 26.88 & 25.02 & 20.63 & \textbf{26.88} & 26.80 & \textbf{26.88} & 26.80 & \textbf{26.88} & \textbf{26.88} & 20.41 & \textbf{26.88} \\
    2018-06-30 & 23 & 1000 & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} & \textbf{37.72} \\
    2018-07-22 & 883 & 44 & 92.26 & 15.82 & 22.07 & \textbf{37.62} & 19.14 & 36.97 & 24.32 & 36.08 & 30.93 & 21.98 & 33.59 \\
    2018-07-24 & 400 & 30 & 49.36 & 22.87 & 10.90 & \textbf{35.90} & 25.08 & 32.69 & 27.72 & 31.09 & 31.66 & 10.84 & 29.68 \\
    2018-08-08 & 336 & 38 & 28.53 & 14.72 & 5.15 & \textbf{20.71} & 13.40 & 17.98 & 14.11 & 17.72 & 15.45 & 5.16 & 15.84 \\
    2018-08-18 & 33 & 31 & 0.62 & 0.05 & 0.01 & 0.01 & 0.06 & 0.01 & \textbf{0.07} & 0 & 0 & 0.01 & 0.01 \\
    2018-09-04 & 0 & 30 & 0 & - & - & - & - & - & - & - & - & - & - \\
    2018-09-14 & 2 & 30 & 0.01 & 0 & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & 0 & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} \\
    2018-10-02 & 7 & 600 & 1.21 & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} & \textbf{1.20} \\
    2018-10-17 & 122 & 30 & 14.89 & 2.52 & 2.88 & 3.78 & 2.20 & \textbf{4.71} & 1.95 & 3.71 & 1.89 & 2.88 & 3.13 \\
    2018-11-02 & 715 & 61 & 295.17 & 26.55 & 23.01 & 28.78 & 28 & \textbf{29.52} & 27.80 & 27.46 & 23.84 & 20.80 & 26.78 \\
    2018-11-13 & 100 & 624 & 87.32 & 85.64 & 83.22 & 86.11 & 86.11 & \textbf{86.50} & 86.11 & 86.47 & 84.01 & 82.24 & 83.05 \\
    2018-12-01 & 115 & 1000 & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} & \textbf{18.43} \\
    2018-12-27 & 123 & 1000 & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} & \textbf{22.15} \\
    \midrule
    Total & 6037 & 9102 & 2180.77 & 1483.34 & 1463.54 & \textbf{1537.55} & 1494.10 & 1520.72 & 1500.52 & 1506.31 & 1502.74 & 1458.10 & 1509.89 \\
    Avg. & 241.48 & 364.08 & 87.23 & 59.33 & 58.54 & \textbf{61.50} & 59.76 & 60.83 & 60.02 & 60.25 & 60.11 & 58.32 & 60.40 \\
    \bottomrule
    \end{tabular}
    \label{sm:aggZonalCurtail}
\end{table}

